ER-Test: Evaluating Explanation Regularization Methods for Language Models

By explaining how humans would solve a given task, human rationales can provide strong learning signal for neural language models (LMs). Explanation regularization (ER) aims to improve LM generalization by pushing the LM's machine rationales (Which input tokens did the LM focus on?) to align with human rationales (Which input tokens would humans focus on?). Though prior works primarily study ER via in-distribution (ID) evaluation, out-of-distribution (OOD) generalization is often more critical in real-world scenarios, yet ER's effect on OOD generalization has been underexplored. In this paper, we introduce ER-Test, a framework for evaluating ER models' OOD generalization along three dimensions: unseen dataset tests, contrast set tests, and functional tests. Using ER-Test, we extensively analyze how ER models' OOD generalization varies with different ER design choices. Across two tasks and six datasets, ER-Test shows that ER has little impact on ID performance but can yield large OOD performance gains. Also, we find that ER can improve OOD performance even with limited rationale supervision. ER-Test's results help demonstrate ER's utility and establish best practices for using ER effectively.

==> sections/9_discussion_future_work.tex <==
\section{Conclusion and Future Work} 
\label{sec:discussion_future_work}
% \vspace{-0.2cm}

% \brihi{complete this}
% \xiang{re-purpose to be conclusion and future work. Can point to a detailed version in appendix}

\aaron{Update this}

In this work, we study explanation regularization (ER) -- aligning machine rationales with human rationales, in detail. We propose \method, that evaluates ER's OOD generalization along three pillars - unseen datasets, contrast set tests and functional tests, and uses it to investigate four research questions surrounding the choice of the rationale alignment criterion, type of human rationale, choice of and time taken to obtain rationale-annotation instances. Although ER shows minor impact on ID task performance, improvements on OOD datasets is significant. Furthermore, ER not only works well with dense, instance-level human rationales, but also with distantly supervised task-level rationales. Lastly, ER is shown to provide benefits even with limited number of rationale-annotated instances, or within time constraints for rationale annotation. In future, we aim to study ER as a tool for improving human-in-the-loop (HITL) debugging of LMs. Furthermore, currently \method is only defined for extractive rationales. Human feedback for free-text machine rationales is also a promising extension for \method.

% \paragraph{Online ER and connections to human-in-the-loop learning} Fine-tuning strategies have shown to distort the underlying data distribution \cite{kumar2022finetuning}, therefore, once $\mathcal{F}$ undergoes ER, its machine rationales differ from before. Currently, ER is being studied in an offline manner -- once human rationales are collected, they are used to update model weights. However, what is more effective is to study the effect of ER when applied incrementally, thus improving rationale alignment. 




